An Infinite Dimensional Virtual Cohomology Group of $\textbf{SL}_3(\mathbb{Z}[t])$

We prove that $\textbf{SL}_3(\mathbb{Z}[t])$ has a finite index subgroup $\Gamma$ such that $H^2(\Gamma; \mathbb{Q})$ is infinite dimensional. The proof uses the geometry of the Euclidean building for $\textbf{SL}_3(\mathbb{Q}((t^{-1})))$.

==> ContentFiles/CongruenceSubgroups/Wrapper.tex <==
\chapter[A Sequence of Subgroups of $U(\textbf{SL}_3(\Q\lbrack t\rbrack))$]
	{A Sequence of Subgroups of $U(\textbf{SL}_3(\Q\lbrack t\rbrack))$}
\chaptermark{A Sequence of Subgroups of $U(\textbf{SL}_3(\Q\lbrack t\rbrack))$}

\input{ContentFiles/CongruenceSubgroups/CongruenceSubgroupsContent}
%{A sequence of subgroups of $U(\SL_3(\Q[t]))$}

==> ContentFiles/ConnectedComplex/Wrapper.tex <==
\chapter[Construction of a $2$-connected $\Gamma$-complex]
        {Construction of a $2$-connected $\Gamma$-complex}
\chaptermark{Construction of a $2$-connected $\Gamma$-complex}
\label{sec:connectedComplex}

\input{ContentFiles/ConnectedComplex/TopOfConnectedComplex}

\section{$\Gamma\setminus X_0$ Is Contractible}
\input{ContentFiles/ConnectedComplex/Contractibility}

==> ContentFiles/GlobalCocycles/Wrapper.tex <==
\chapter[A Family of Global Cocycles]
        {A Family of Global Cocycles}
\chaptermark{A Family of Global Cocycles}
\label{sec:globalCocycles}

\input{ContentFiles/GlobalCocycles/top}

\section{A Function on Global Disks}
\input{ContentFiles/GlobalCocycles/FunctionOnGlobalDisksSubContent}

\section{A $2$-cochain on $\Gamma\setminus Y$}
\input{ContentFiles/GlobalCocycles/2CoChainSubSection}

\section{A Sequence of Cycles}
\input{ContentFiles/GlobalCocycles/SequenceOfCyclesSubSection}

\subsection{A Free Subgroup of $\SL_2(\Z[t])$}
\input{ContentFiles/GlobalCocycles/FreeSubgroupSubSection}

\subsection{A Small Unipotent Toolkit}
\input{ContentFiles/GlobalCocycles/SmallUnipotentToolkit}

\subsection{A Subspace of the `Boundary' of the Standard Sector}
\input{ContentFiles/GlobalCocycles/SubSpaceOfBoundarySubSection}

\subsection{The Global Disk}
\input{ContentFiles/GlobalCocycles/TheGlobalDiskSubSection}

\subsection{Turning Global Disks Into Quotient Cycles}
\input{ContentFiles/GlobalCocycles/TurningGlobalDisksIntoQuotientCyclesSubSection}

==> ContentFiles/Introduction/Cohomology_Review.tex <==


We begin with a brief review of what it means to take the cohomology of a group with coefficients. A good reference with more detail is \cite{Br}.  

==> ContentFiles/Introduction/Wrapper.tex <==
\chapter[Introduction]
        {Introduction}
\chaptermark{Introduction}

\input{ContentFiles/Introduction/TopOfIntro}


\section{Outline of Paper}
\input{ContentFiles/Introduction/OutlineOfPaper}

==> ContentFiles/LocalCocycles/Wrapper.tex <==
\chapter[Local Cocycles]
        {Local Cocycles}
\chaptermark{Local Cocycles}
\label{sec:localCocycles}
\input{ContentFiles/LocalCocycles/TopOfLocalCocycles}

\section{A Local Cycle Which Evaluates to Be Nonzero}
\input{ContentFiles/LocalCocycles/NonzeroCycle}

==> ContentFiles/LocalStars/Wrapper.tex <==
\chapter[Stars About Vertices in $\Sect$]
        {Stars About Vertices in $\Sect$}
\chaptermark{Stars About Vertices in $\Sect$}

\input{ContentFiles/LocalStars/LocalStarsContent}

==> ContentFiles/MainProof/Wrapper.tex <==
\chapter[Proof of the Main Theorem]
        {Proof of the Main Theorem}
\chaptermark{Proof of the Main Theorem}

\input{ContentFiles/MainProof/MainProofContent}

==> ContentFiles/Preliminaries/Wrapper.tex <==
\chapter[Preliminaries]
        {Preliminaries}
\chaptermark{Preliminaries}

\input{ContentFiles/Preliminaries/PreliminariesContent}

==> ContentFiles/ReducingDisks/Wrapper.tex <==
\chapter[Reducing Disks in $X$]
        {Reducing Disks in $X$}
\chaptermark{Reducing Disks in $X$}

\input{ContentFiles/ReducingDisks/ReducingDisksContent}

==> ContentFiles/SequenceOfVertices/Wrapper.tex <==
\chapter[A Sequence of Vertices in $\Sect$]
        {A Sequence of Vertices in $\Sect$}
\chaptermark{A Sequence of Vertices in $\Sect$}

\input{ContentFiles/SequenceOfVertices/SequenceOfVerticesContent}
